Refined $\alpha$-Divergence Variational Inference via Rejection Sampling

We present an approximate inference method, based on a synergistic combination of R\'enyi $\alpha$-divergence variational inference (RDVI) and rejection sampling (RS). RDVI is based on minimization of R\'enyi $\alpha$-divergence $D_\alpha(p||q)$ between the true distribution $p(x)$ and a variational approximation $q(x)$; RS draws samples from a distribution $p(x) = \tilde{p}(x)/Z_{p}$ using a proposal $q(x)$, s.t. $Mq(x) \geq \tilde{p}(x), \forall x$. Our inference method is based on a crucial observation that $D_\infty(p||q)$ equals $\log M(\theta)$ where $M(\theta)$ is the optimal value of the RS constant for a given proposal $q_\theta(x)$. This enables us to develop a \emph{two-stage} hybrid inference algorithm. Stage-1 performs RDVI to learn $q_\theta$ by minimizing an estimator of $D_\alpha(p||q)$, and uses the learned $q_\theta$ to find an (approximately) optimal $\tilde{M}(\theta)$. Stage-2 performs RS using the constant $\tilde{M}(\theta)$ to improve the approximate distribution $q_\theta$ and obtain a sample-based approximation. We prove that this two-stage method allows us to learn considerably more accurate approximations of the target distribution as compared to RDVI. We demonstrate our method's efficacy via several experiments on synthetic and real datasets.

==> intro.tex <==
  We present an  approximate inference method, based on a synergistic combination of R\'enyi $\alpha$-divergence variational inference (RDVI) and rejection sampling (RS). RDVI is based on minimization of R\'enyi $\alpha$-divergence $D_\alpha(p||q)$ between the true distribution $p(x)$ and a variational approximation $q(x)$; RS draws samples from a distribution $p(x) = \tilde{p}(x)/Z_{p}$ using a proposal $q(x)$, s.t. $Mq(x) \geq \tilde{p}(x), \forall x$. Our inference method is based on a crucial observation that $D_\infty(p||q)$ equals $\log M(\theta)$ where $M(\theta)$ is the optimal value of the RS constant for a given proposal $q_\theta(x)$. This enables us to develop a \emph{two-stage} hybrid inference algorithm.% Stage-1 performs RDVI to learn $q_\theta$ by minimizing an estimator of $D_\alpha(p||q)$, and uses the learned $q_\theta$ to find an (approximately) optimal $\tilde{M}(\theta)$. Stage-2 performs RS using the constant $\tilde{M}(\theta)$ to improve the approximate distribution $q_\theta$ and obtain a sample-based approximation.
  
There is an increasing interest in developing more expressive variational posteriors for (shallow/deep) latent variable models and Bayesian neural networks~\cite{rezende2015variational,salimans2015markov,chen2016variational}. In particular, the combination of MCMC and variational methods has been used in recent work to learn expressive variational posteriors ~\cite{salimans2015markov} having the best of both worlds. Rejection Sampling~\cite{bishop2006pattern}, which we use as a subroutine (with learned $M$) in our algorithm $\alpha$-DRS, is a popular sampling technique that generates independent samples from a complex distribution indirectly through a simple distribution. In addition to being a useful sampling algorithm in its own right, recently \emph{approximations} of Rejection Sampling have also been used for designing variational inference algorithms. In particular, Variational Rejection Sampling (VRS) ~\cite{grover2018variational} which uses rejection sampling to learn a better variational approximation. Recently Rejection sampling has also been used to improve the generated samples from GAN (Generative Adversarial Nets)~\cite{azadi2018discriminator} and improve priors for variational inference ~\cite{bauer2018resampled}.

